The Role of Context in Detecting Previously Fact-Checked Claims

Recent years have seen the proliferation of disinformation and fake news online. Traditional approaches to mitigate these issues is to use manual or automatic fact-checking. Recently, another approach has emerged: checking whether the input claim has previously been fact-checked, which can be done automatically, and thus fast, while also offering credibility and explainability, thanks to the human fact-checking and explanations in the associated fact-checking article. Here, we focus on claims made in a political debate and we study the impact of modeling the context of the claim: both on the source side, i.e., in the debate, as well as on the target side, i.e., in the fact-checking explanation document. We do this by modeling the local context, the global context, as well as by means of co-reference resolution, and multi-hop reasoning over the sentences of the document describing the fact-checked claim. The experimental results show that each of these represents a valuable information source, but that modeling the source-side context is most important, and can yield 10+ points of absolute improvement over a state-of-the-art model.

==> sections/supplemental_material.tex <==
\section{Experimental Details}

\paragraph{Hyper-parameters}

$FC(3,1)$:

top-3 sentences

top-100 sentences

pre-training on FEVER, 

\textbf{Rank-SVM:}  

\textbf{BM25}\cite{robertson2009probabilistic}: It is a classical approach in information retrieval. It assigns a score to each query-document pair based on exact matching between the words in the query and the words in a target document, and it uses this score for ranking.

